Revising Properties of Planet-Host Binary Systems. III. There is No Observed Radius Gap For Kepler Planets in Binary Star Systems

Binary stars are ubiquitous; the majority of solar-type stars exist in binaries. Exoplanet occurrence rate is suppressed in binaries, but some multiples do still host planets. Binaries cause observational biases in planet parameters, with undetected multiplicity causing transiting planets to appear smaller than they truly are. We have analyzed the properties of a sample of 119 planet-host binary stars from the Kepler mission to study the underlying population of planets in binaries that fall in and around the radius valley, which is a demographic feature in period-radius space that marks the transition from predominantly rocky to predominantly gaseous planets. We found no statistically significant evidence for a radius gap for our sample of 122 planets in binaries when assuming the primary stars are the planet hosts, with a low probability ($p < 0.05$) of the binary planet sample radius distribution being consistent with the single-star small planet population via an Anderson-Darling test. These results reveal demographic differences in the planet size distribution between planets in binary and single stars for the first time, showing that stellar multiplicity may fundamentally alter the planet formation process. A larger sample and further assessment of circumprimary versus circumsecondary transits is needed to either validate this non-detection or explore other scenarios, such as a radius gap with a location that is dependent on binary separation.

==> excluded_systems.tex <==
KOI-0126 &	Quad\\
KOI-0279 &	Triple\\
KOI-0307 &	Quad\\
KOI-0353 &	Triple\\
KOI-0364 &	Quad\\
KOI-0387 &	Triple\\
KOI-0442 &	Possible single\\
KOI-0511 &	Quad\\
KOI-0658 &	Triple\\
KOI-0854 &	Triple\\
KOI-0984 &	Triple\\
KOI-0987 &	Quad\\
KOI-1151 &	Triple\\
KOI-1361 &	Triple\\
KOI-1397 &	High-order multiple\\
KOI-1531 &	Triple\\
KOI-1537 &	Single\\
KOI-1589 &	High-order multiple\\
KOI-1615 &	Quad\\
KOI-1660 &	Triple\\
KOI-1890 &	Triple\\
KOI-1908 &	Triple\\
KOI-1961 &	Triple\\
KOI-2009 &	Triple\\
KOI-2031 &	Triple\\
KOI-2091 &	Too hot for models\\
KOI-2159 &	High-order multiple\\
KOI-2174 &	High-order multiple\\
KOI-2421 &	High-order multiple\\
KOI-2554 &	Triple\\
KOI-2641 &	Quad\\
KOI-2705 &	Triple\\
KOI-2733 &	Triple\\
KOI-2797 &	Single?\\
KOI-2904 &	Too hot for models\\
KOI-2927 &	Triple\\
KOI-2971 &	Quad\\
KOI-3029 &	Quad\\
KOI-3049 &	Quad\\
KOI-3073 &	Triple\\
KOI-3136 &	Triple\\
KOI-3284 &	Triple\\
KOI-3349 &	Triple\\
KOI-3377 &	Triple\\
KOI-3415 &	Triple\\
KOI-3444 &	Triple\\
KOI-3480 &	Triple\\
KOI-3497 &	Triple\\
KOI-4021 &  Possible giant\\
KOI-4184 &	Triple\\
KOI-4208 &	Quad\\
KOI-4209 &	Background star\\
KOI-4287 &	Quad\\
KOI-4323 &	Quad\\
KOI-4329 &	Triple\\
KOI-4343 &	Quad\\
KOI-4399 &	Quad\\
KOI-4550 &	Triple\\
KOI-4567 &	Quad\\
KOI-4634 &	Triple\\
KOI-4651 &	Triple\\
KOI-4653 &	Single\\
KOI-4713 &	Triple\\
KOI-4759 &	Triple\\
KOI-4871 &	Triple\\
KOI-5327 &	Quad\\
KOI-5570 &	Triple\\
KOI-5762 &	Triple\\
KOI-6513 &	Quad\\
KOI-6610 &	Triple\\
KOI-7470 &	Triple\\
